Charge-dependent slip flow of ionic liquids through the non-uniform microfluidic device: pressure drop and electroviscous effects

This work investigates electroviscous effects in presence of charge-dependent slip in steady pressure-driven laminar flow of a symmetric (1:1) electrolyte liquid through a uniformly charged slit contraction - expansion (4:1:4) microfluidic device. The mathematical model comprising Poisson's, Nernst-Planck, Navier-Stokes, and current continuity equations are solved numerically using finite element method (FEM). The flow fields (electrical potential, charge, induced electric field strength, pressure drop, and electroviscous correction factor) have been obtained and presented for a wide range of parameters like inverse Debye length (K=2-20), surface charge density (S=4-16) and slip length ($0\le B_0\le 0.20$) at fixed Schmidt number (Sc=1000) and low Reynolds number (Re=0.01). The flow fields have shown complex dependence on governing parameters. The charge-dependent slip has further enhanced complexity of dependency in comparison to no-slip condition. The total electrical potential ($|\Delta U|$) maximally increases by 78.68%, and pressure drop ($|\Delta P|$) maximally decreases by 63.42%, relative to no-slip flow, over the ranges of conditions. The electroviscous correction factor ($Y=$ ratio of apparent to physical viscosity) increases by 33.58% under the no-slip ($B_0=0$) condition. It ($Y$) increases maximally by 72.10% for charge-dependent slip than in no-slip flow for considered ranges of the conditions. A simple analytical model to estimate the pressure drop in the electroviscous flow has been developed based on the Poiseuille flow in individual uniform sections and pressure loss due to thin orifice. The model overpredicts pressure drop by 2 - 4% from the numerical values. Finally, the predictive relations, depicting the functional dependence of numerical results on governing parameters, are presented for their practical use in design and engineering of microfluidic devices.

==> Makefile <==
# type "make" command in Unix to create ps and pdf file 
#
#Colors
gray=\e[1;30m
red=\e[0;31m
RED=\e[1;31m
blue=\e[0;34m
BLUE=\e[1;34m
green=\e[0;32m
GREEN=\e[1;32m
cyan=\e[0;36m
CYAN=\e[1;36m
NC=\e[0m # No Color

# the documents to be compiled by default
# set defaultfile to the name of the main file without the .tex
#
defaultfile = $(foreach i,$(filter-out ,$(shell grep -l documentclass *.tex)), $(basename $i))
#
ASPELL = aspell -t -c --mode=tex
ISPELL = ispell -t  --mode=tex
LATEX = latex -interaction=batchmode
BIBTEX = bibtex 
MAKEINDEX = makeindex
PDFLATEX = pdflatex -interaction=batchmode
#
DVIPS = dvips -Pwww
DVIPDF = dvipdf 
PSPDF = ps2pdf
#
all: pdf clean
#
pdf:
	@echo -e ""
	@echo -e "$(BLUE)====> Default file being compiled: $(RED)$(defaultfile).tex$(NC)"
	@echo -e ""
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running BibTex$(NC)" ;
	$(BIBTEX) $< $(QUIET)$(defaultfile)
#	
#	@echo -e "$(BLUE)====> $(green)Running aspell$(NC)" ;
#	$(ASPELL) $< $(QUIET)$(defaultfile).tex
#
#	@echo -e "$(BLUE)====> $(green)Running ispell$(NC)" ;
#	$(ISPELL) $< $(QUIET)$(defaultfile).tex
#
	@echo -e "$(BLUE)====> $(green)Running Makeindex$(NC)" ;
	$(MAKEINDEX) $< $(QUIET)$(defaultfile).nlo -s nomencl.ist -o  $(QUIET)$(defaultfile).nls
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Running PDFLaTeX to generate PDF document$(NC)" ;
#	$(PDFLATEX) $< $(QUIET)$(defaultfile)
#
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Running LaTeX$(NC)" ;
	$(LATEX) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PS document from DVI document$(NC)" ;
	$(DVIPS) $< $(QUIET)$(defaultfile)
#
	@echo -e "$(BLUE)====> $(green)Generating PDF document from DVI document$(NC)" ;
	$(DVIPDF) $< $(QUIET)$(defaultfile)
#
#	@echo -e "$(BLUE)====> $(green)Generating PDF document from PS document$(NC)" ;
#	$(PSPDF) $(defaultfile).ps $(defaultfile).pdf
#
clean:
	@echo -e "$(RED)====> $(red)Cleaning up temporary files$(NC)"
	rm -f *.brf *.glo *.ist *.nlo  *.out *.spl *.log *.aux *.*% *.lof *.gls *.nls
	rm -f *.lop *.lot *.toc *.idx *.ilg *.ind *.bbl *.blg *.backup *.bak *~



